FollowTable: A Benchmark for Instruction-Following Table Retrieval

Table Retrieval (TR) has traditionally been formulated as an ad-hoc retrieval problem, where relevance is primarily determined by topical semantic similarity. With the growing adoption of LLM-based agentic systems, access to structured data is increasingly instruction-driven, where relevance is conditional on explicit content and schema constraints rather than topical similarity alone. We therefore formalize Instruction-Following Table Retrieval (IFTR), a new task that requires models to jointly satisfy topical relevance and fine-grained instruction constraints. We identify two core challenges in IFTR: (i) sensitivity to content scope, such as inclusion and exclusion constraints, and (ii) awareness of schema-grounded requirements, including column semantics and representation granularity--capabilities largely absent in existing retrievers. To support systematic evaluation, we introduce FollowTable, the first large-scale benchmark for IFTR, constructed via a taxonomy-driven annotation pipeline. We further propose a new metric, termed the Instruction Responsiveness Score, to evaluate whether retrieval rankings consistently adapt to user instructions relative to a topic-only baseline. Our results indicate that existing retrieval models struggle to follow fine-grained instructions over tabular data. In particular, they exhibit systematic biases toward surface-level semantic cues and remain limited in handling schema-grounded constraints, highlighting substantial room for future improvements.

==> tables/breakdown.tex <==
\caption{Fine-grained performance breakdown across the five instruction types defined in our taxonomy. 
\textbf{C1--C2} denote Content-scope constraints (Explicit Boundary, Exclusive Scope), while \textbf{S1--S3} denote Schema-grounded constraints (Attribute, Entity, Granularity). 
For each type, we report nDCG@10 on instruction queries (\textbf{Ins.}) and ICRC.}
\label{table:fine_grained_results}
\centering

\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}

\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}
& \multicolumn{2}{c}{\textbf{C1: Explicit Boundary}}
& \multicolumn{2}{c}{\textbf{C2: Exclusive Scope}}
& \multicolumn{2}{c}{\textbf{S1: Attribute-Focus}}
& \multicolumn{2}{c}{\textbf{S2: Entity-Centric}}
& \multicolumn{2}{c}{\textbf{S3: Granularity}} \\

\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}

& nDCG. $\uparrow$ & IRS $\uparrow$
& nDCG. $\uparrow$ & IRS $\uparrow$
& nDCG. $\uparrow$ & IRS $\uparrow$
& nDCG. $\uparrow$ & IRS $\uparrow$
& nDCG. $\uparrow$ & IRS $\uparrow$ \\

\midrule
\multicolumn{11}{c}{\textit{\textbf{No-Instruction Retrievers}}} \\
\midrule

BM25        & 46.9 & 12.6 & 30.5 & -1.3 & 20.1 & -6.4 & 32.4 & 7.7 & 27.1 & 7.0 \\
e5-large-v2   &   &   &   &   &   &   &   &   &   &   \\
Tapas       & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0 \\
Qwen-Emb-8B & 83.3  & 30.9 & 71.5  & 23.4 & 75.1  & 16.5 & 67.7  & 17.1 & 65.0  & 18.2 \\
promptriever & 84.3  & 36.7 & 69.3  & 24.8 & 75.5  & 25.1 & 68.7  & 20.8 & 68.0  & 22.9 \\
FollowIR & 86.1  & 56.3 & 76.9  & 38.7 & 77.7  & 35.8 & 71.6  & 30.3 & 73.1  & 39.6 \\

\bottomrule
\end{tabular}%
}

